Context Matters: Graph-based Self-supervised Representation Learning for Medical Images

Supervised learning method requires a large volume of annotated datasets. Collecting such datasets is time-consuming and expensive. Until now, very few annotated COVID-19 imaging datasets are available. Although self-supervised learning enables us to bootstrap the training by exploiting unlabeled data, the generic self-supervised methods for natural images do not sufficiently incorporate the context. For medical images, a desirable method should be sensitive enough to detect deviation from normal-appearing tissue of each anatomical region; here, anatomy is the context. We introduce a novel approach with two levels of self-supervised representation learning objectives: one on the regional anatomical level and another on the patient-level. We use graph neural networks to incorporate the relationship between different anatomical regions. The structure of the graph is informed by anatomical correspondences between each patient and an anatomical atlas. In addition, the graph representation has the advantage of handling any arbitrarily sized image in full resolution. Experiments on large-scale Computer Tomography (CT) datasets of lung images show that our approach compares favorably to baseline methods that do not account for the context. We use the learnt embedding to quantify the clinical progression of COVID-19 and show that our method generalizes well to COVID-19 patients from different hospitals. Qualitative results suggest that our model can identify clinically relevant regions in the images.

==> conclusion.tex <==
In this paper, we introduce a novel method for unsupervised representation learning in volumetric medical images. We represent 3D image as a graph of patches with anatomical consistence. In addition, we introduced a multi-scale model which includes a conditional encoder for local textural and spatial feature extraction and a graph convolutional network for global contextual feature extraction, which indicates that our model focus on clinical-relevant regions. In addition, we propose a task-specific method for model explanation. The experiments on multiple datasets demonstrate that our proposed method is effective, robust and generalizable.

==> experiments.tex <==
We evaluate the performance of the proposed model on two large-scale datasets of 3D medical images. We compare our model with various baseline methods, including both supervised approaches: Subject2Vec~\cite{singla2018subject2vec},  Slice-based CNN~\cite{gonzalez2018disease}, and unsupervised approaches: MoCo~\cite{he2020momentum}, LLE~\cite{schabdach2017likelihood}, K-means algorithm applied to image features extracted from local lung regions~\cite{schabdach2017likelihood}, and Low Attenuation Area (LAA) features.

\subsection{Datasets}

The experiments are conducted on three large-scale volumetric medical imaging datasets, including the COPDGene dataset~\cite{regan2011genetic}, the MosMedData dataset~\cite{morozov2020MosMedData} and the COVID-19 CT dataset.

%{\vspace{2mm} \par \bf \noindent COPDGene Dataset: \hspace{2mm}}
\subsubsection{COPDGene Dataset}
We use 3D thorax computerized tomography (CT) images of 9,180 subjects from COPDGene dataset in our study. The images are re-sampled to isotropic $1 mm^3$ resolution. The Hounsfield Units (HU) are mapped to the intensity window of $[-1024,240]$ and normalized to $[-1,1]$. 

\subsubsection{MosMedData Dataset}
We use 3D CT scans of 1,110 subjects from the MosMedData dataset~\cite{morozov2020MosMedData} in our study. The images are categorized into five classes based on severity of lung tissue abnormalities with COVID-19. we re-sampled the images to isotropic $1 mm^3$ resolution. The Hounsfield Units (HU) are mapped to the intensity window of $[-1024,240]$ and normalized to $[-1,1]$. 

%{\vspace{2mm} \par \bf \noindent COVID-19 Dataset: \hspace{2mm} }
\subsubsection{COVID-19 CT Dataset}
We collect a multi-hospital 3D thorax CT images on COVID-19 consisted of 80 subjects. The 35 positive subjects are come from multiple publicly released COVID-19 dataset~\cite{COVID-19-SegBenchmark,segcovid,zhou2020rapid}. We randomly sample 45 healthy subjects in LIDC-IDRI dataset~\cite{armato2011lung} as negative samples.
We resample all images to $1 mm^3$
isotropic resolution. The Hounsfield Units (HU) are mapped to the intensity window of $[-1024,240]$ and normalized to $[-1,1]$.

\subsection{Quantitative Evaluation}
We evaluate the performance of proposed method by using extracted representations of subjects to predict clinical-relevant variables. 

\subsubsection{COPDGene dataset}
We first perform unsupervised pre-training on COPDGene dataset. Then we freeze the features and train a linear regression model to predict the {\it logarithm} of the two continuous clinical variables, including percent predicted values of Forced Expiratory Volume in one second (\texttt{FEV1pp}) and its ratio with Forced vital capacity (FVC) (\texttt{$\text{FEV}_1 / \text{FVC}$}). We report average of the $R^2$ scores in five-fold cross-validation.
We train a logistic regression model for each of the six categorical variables, including (1) Global Initiative for Chronic Obstructive Lung Disease (\texttt{GOLD}) score, which is a four-grade categorical value indicating the severity of airflow limitation, (2) Centrilobular emphysema (\texttt{CLE}) visual score, which is a six-grade categorical value indicating the severity of emphysema in centrilobular, (3) Paraseptal emphysema (\texttt{Para-septal}) visual score, which is a three-grade categorical value indicating the severity of paraseptal emphysema, (4) Acute Exacerbation history (\texttt{AE history}), which is a binary variable indicating whether the subject has experienced at least one exacerbation before enrolling in the study, (5) Future Acute Exacerbation (\texttt{Future AE}), which is a binary variable indicating whether the subject has reported experiencing at least one exacerbation at the 5-year longitudinal follow up, (6) Medical Research Council Dyspnea Score (\texttt{mMRC}), which is a five-grade categorical value indicating dyspnea symptom.
The evaluation results on COPDGene dataset are shown in Table~\ref{tbl:COPD}. For all results, we report average test accuracy in five-fold cross-validation.
\begin{table*}[t]
 \centering
 %\vspace{-3mm}
 \caption{ Evaluation on COPD dataset}
 \label{tbl:COPD}
  \begin{tabular}{lccccccccc}
  \toprule
   Method&Supervised&$\log$\texttt{FEV1pp}&$\log$\texttt{$\text{FEV}_1 / \text{FVC}$}&GOLD&CLE&Para-septal&AE History&Future AE&mMRC\\
   \toprule
   Metric&  &\multicolumn{2}{c}{R-Square}& \multicolumn{6}{c}{\% Accuracy}  \\
   \midrule
 LAA-950 &\xmark&0.44$\pm$0.02&0.60$\pm$0.01&55.8&32.9&33.3&73.8&73.8&41.6\\
 K-Means &\xmark&0.55$\pm$0.03&0.68$\pm$0.02&57.3&-&-&-&-&-\\
 LLE &\xmark& 0.58$\pm$0.03&0.70$\pm$0.02&58.9&-&-&-&-&-\\
 ModelsGenesis&\xmark&0.58$\pm$0.01&0.64$\pm$0.01&59.5&41.8&52.7&77.8&76.7&46.0\\
 MoCo &\xmark& 0.40$\pm$0.02&0.49$\pm$0.02&52.7&36.5&52.5&78.6&\textbf{82.0}&46.4\\
 \midrule
2D CNN &\cmark&0.53&-&51.1&-&-&60.4&-&-\\
Subject2Vec &\cmark&\textbf{0.67$\pm$0.03}&\textbf{0.74$\pm$0.01}&\textbf{65.4}&40.6&52.8&76.9&68.3&43.6\\
 \midrule
 Ours w/o CE&\xmark&0.56$\pm$0.03&0.65$\pm$0.03&61.6&48.1&55.5&\textbf{78.8}&80.8&50.4\\
 Ours w/o Graph&\xmark&0.60$\pm$0.01&0.69$\pm$0.01&62.5&49.2&55.8&78.7&80.7&50.6\\
 Ours&\xmark&0.62$\pm$0.01&0.70$\pm$0.01&63.2&\textbf{50.4}&\textbf{56.2}&\textbf{78.8}&81.1&\textbf{51.0}\\
  \bottomrule
   \multicolumn{10}{p{.5\textwidth}}{- indicates not reported.}
  \end{tabular}
 % \vspace{-3mm}
 \end{table*}
 
 The results show that our proposed model outperforms baseline unsupervised methods in all metrics except for \texttt{Future AE}. While MoCo is also a contrastive learning based method, we believe that our proposed method achieves better performance due to two reasons: (1) Since MoCo can only accept fixed-size input, we resize all volumetric images into $256\times256\times256$. In this way, some lungs may have been distorted and fine-details are lost due to down-sampling. In comparison, our model natively supports arbitrary sized images in full resolution. (2) Since training CNN model with volumetric images is extremely memory-intensive, we can only set the batch size as 4 at most when training the MoCo model, the small batch size may lead to unstable gradient. In comparison, the interleaving training scheme reduces memory footprint and enables our model to train using a larger batch size.
 
Our method also outperforms supervised methods, including Subject2Vec and 2D CNN, in terms of \texttt{CLE}, \texttt{Para-septal}, \texttt{AE History}, \texttt{Future AE} and \texttt{mMRC}; for other features, the performance gap is smaller than other unsupervised methods. We believe that the performance improvement our graph-based representation. Subject2Vec uses a unordered set-based representation which may not account for spatial locations of the patches. 2D CNN only uses 2D slices which may not leverage information in 3D structure. Overall, he results imply that representation extracted by our model preserves more information about the disease severity than baselines.
 
 \subsubsection{MosMedData dataset}
 We first perform unsupervised pre-training on MosMedData dataset. Then we freeze the features and train a logistic regression model to predict the severity of lung tissue abnormalities with COVID-19 based on CT finding and clinical data, which is a five-grade categorical value. The evaluation results on MosMedData dataset are shown in Table~\ref{tbl:RU}. For all results, we report average test accuracy and the percentage of the times the predicted class laid within one class of true value (one-off) in five-fold cross-validation. 
 
 \begin{table}[t]
 \centering
 %\vspace{-3mm}
 \caption{ Evaluation on MosMedData dataset}
 \label{tbl:RU}
  \begin{tabular}{lccc}
  \toprule
   Method&Supervised&\% Acc&\% Acc one-off\\
   \midrule
ModelsGenesis &\xmark&62.1&95.6\\
MoCo &\xmark&62.1&95.6\\
3D CNN &\cmark&61.2&95.6\\
 \midrule
 Ours w/o CE&\xmark&63.3&\textbf{96.2}\\
Ours w/o Graph&\xmark&64.3&96.1\\
Ours&\xmark&\textbf{65.3}&\textbf{96.2}\\
  \bottomrule
  \end{tabular}
 % \vspace{-3mm}
 \end{table}

 The results show that our proposed model outperforms both unsupervised MoCo model and supervised 3D CNN model. We believe that our unsupervised model outperforms supervised 3D CNN model in this case is due to limited annotated data available. A supervised model may not converge well or easily become overfitted. In comparison, a supervised model is not likely to become overfitted due to the contrastive learning objective. The results imply that our model is more robust and learns better representation than supervised method when limited data is available.
 
\subsubsection{COVID-19 CT Dataset}
Since the size of COVID-19 CT Dataset is small (only 80 images are available), we don't directly train our unsupervised model on this dataset. Instead, we use models pre-trained on COPDGene and MosMedData dataset to extract feature from COVID-19 CT Dataset, respectively. Then we train a logistic regression model to predict whether the CT scan comes from a COVID-19 patient. The evaluation results are shown in Table~\ref{tbl:COVID}. We report average test accuracy and area under the ROC curve (AUROC) in five-fold cross-validation. 

 \begin{table*}[t]
 \centering
 %\vspace{-3mm}
 \caption{ Evaluation on COVID-19 CT dataset}
 \label{tbl:COVID}
  \begin{tabular}{lccc}
  \toprule
   Method&Supervised&\% Acc&AUROC\\
   \midrule
MoCo (Pretrained on COPDGene) &\xmark&75.0&0.855\\
MoCo (Pretrained on MosMedData) &\xmark&86.3&0.935\\
3D CNN &\cmark&68.8&0.821\\
 \midrule
Ours (Pretrained on COPDGene)&\xmark&88.7&\textbf{0.975}\\
Ours (Pretrained on MosMedData)&\xmark&\textbf{91.2}&0.963\\
  \bottomrule
  \end{tabular}
 % \vspace{-3mm}
 \end{table*}
 
 The results show that our proposed model outperforms both unsupervised MoCo model and supervised 3D CNN model. We found that unsupervised models pretrained on MosMedData dataset has a better performance than models pretrained on COPDGene dataset. We speculate that since MosMedData dataset contains subjects with COVID-19 related lung tissue abnormalities (e.g. ground glass opacities), models pertrained on MosMedData dataset learn these relevant features transferred the knowledge when extracting features from COVID-19 dataset. The results demonstrates the robustness and generality of our proposed model, it also implies that our model learns better representation than supervised method when limited data is available.
%.
\subsection{Embedding Visualization}
We use tSNE~\cite{maaten2008visualizing} to visualize subject-level features extracted on COPDGene dataset in two dimension. In Fig~\ref{fig:gold}, we found that subjects with GOLD score of (0,1) and (3,4) are separable under two dimension. But subjects with \texttt{GOLD} score 2 are scattered. It requires further investigation to understanding of embedding pattern of subjects subjects with \texttt{GOLD} score 2. In Fig~\ref{fig:fev1}, we can find a direction along which we can see decreasing \texttt{FEV1pp}.

\begin{figure}[t]
\centering
    \includegraphics[width = .49\textwidth]
    {figures/GOLD.png}
    \caption{Embedding of subjects in 2D using \ky{UMAP}. Each dot represents one subject colored by the \texttt{GOLD} score.  
    }
    \label{fig:gold}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width = .49\textwidth]
    {figures/logFEV1.png}
    \caption{Embedding of subjects in 2D using \ky{UMAP}. Each dot represents one subject colored by $\log$ \texttt{FEV1pp}.  
    }
    \label{fig:fev1}
\end{figure}

\subsection{Model Explanation}
We use the class activation graph method described before to visualize discriminative image regions used by our model for prediction in downstream task. In Fig.~\ref{fig:copd}, we apply the explanation method using the target variable $-\log \texttt{FEV1pp}$ on a $GOLD$ 4 subject in COPDGene dataset, since low $\texttt{FEV1pp}$ value indicates severe disease.  The dark area on the right lung, which is severely damaged, received highest activation value.
In Fig.~\ref{fig:covid}, we apply the explanation method using positive COVID-19 categorical variable on a potivie subject in COVID-19 CT dataset using model pretrained on COPDGene dataset. We can see that the high activation region visualized overlaps with the ground glass opacities, which is a relevant indicator of COVID-19. The results imply that our model has the ability to localize the discriminative image regions.

\begin{figure}[t]
\centering
    \includegraphics[width = .49\textwidth]
    {figures/copd.png}
    \caption{An axial view of the activation map on a $GOLD$ 4 subject in COPDGene dataset. Red color indicate higher relevance to the disease severity.  
    }
    \label{fig:copd}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width = .49\textwidth]
    {figures/covid.png}
    \caption{An axial view of the activation map on a COVID-19 positive subject in COVID-19 CT dataset. Red color indicate higher relevance to the disease severity.  
    }
    \label{fig:covid}
\end{figure}
%\subsection{Image Retrieval}

%\subsection{Ablation Study}

==> introduction.tex <==
While deep neural network trained by the supervised approach has made breakthroughs in many areas, its performance relies heavily on large-scale annotated datasets. Learning informative
%predictive
representation without human-crafted labels has received increased attention in recent years. It has achieved great success in natural language processing~\cite{radford2018improving,devlin2018bert} and computer vision domain~\cite{wu2018unsupervised,chen2020simple,he2020momentum}. In addition, unsupervised learning has the potential for robust and generic representation learning since the features are not optimized towards solving a single supervised task.

%\ky{Annotating large amount of natural images can be done by crowd sourcing~\cite{russakovsky2015imagenet} in a cost-effective manner. However, this approach becomes infeasible in medical imaging because annotation usually requires expert knowledge.} 
Self-supervised learning has emerged as a powerful way of unsupervised learning. It derives input and label from an unlabeled dataset and formulates pretext
%predictive
tasks to train a model. Contrastive learning, a successful example of self-supervised learning, relies on instance discrimination~\cite{wu2018unsupervised} or contrastive predictive coding (CPC)~\cite{oord2018representation}. It has achieved state-of-the-art performance in many aspects~\cite{chen2020simple}. Compared with other self-supervised methods, contrastive learning relies less on heuristics to design pretext tasks. Thus it can learn features of better generality~\cite{chen2020simple}.

There are existing works that focus on self-supervised methods for representation learning in medical imaging. Context restoration~\cite{chen2019self} proposed to learn semantic features by reconstructing images based on corrupted CT images. \cite{taleb2019multimodal} introduced puzzle-solving proxy tasks using multi-modal MRI scans for representation learning. \cite{chaitanya2020contrastive} proposed a local extension of contrastive loss to pre-train model for segmentation using MRI. \cite{taleb2019multimodal} and \cite{chaitanya2020contrastive} down-sampled input images due to memory constraints. However, all these methods use images with fixed dimensions as inputs and cannot extract features at a specific anatomical region.

In this paper, we focus on unsupervised representation learning in volumetric medical imaging, which is a less-explored area. 3D imaging techniques, including computerized tomography (CT) and magnetic resonance images (MRIs), are frequently used in clinical practice to show the 3D anatomy precisely. Comparing with 2D natural images, volumetric medical images have unique properties. First, due to the intrinsic difference between patient subjects, machine types, and operation protocols, image dimension varies across different subjects. As convolutional neural network (CNN) can only handle fixed dimensional input, the common approaches for natural images are to resize the image or crop it to the same dimension. However, both approaches can be problematic for medical images. Taking chest CT for example, reshaping voxels in a CT image may cause distortion in lung, the density for each voxel may get altered too. Cropping images may introduce undesired artifacts as there is a significant variation in the lung volume in population. Second, the size of volumetric medical images is usually large (typically $256\times256\times256$ or larger), as clinicians need high-resolution images to identify subtle lesions, which may consume a huge amount of memory to process. Annotations for medical imaging are also harder to obtain as they need %expertise.
expert knowledge. Self-supervised learning exploiting inherent anatomical information from data is an appealing solution to this problem.


%However, all these methods need to resize the images to a fixed dimension. Due to memory constraints, \cite{taleb2019multimodal} and \cite{chaitanya2020contrastive} down-sampled input images.

%COVID-19 

To address the challenges discussed above, we propose a novel method for unsupervised representation learning in volumetric medical images. We represent a 3D image as a graph of patches with anatomical consistency. Our idea is developed from Subject2Vec~\cite{singla2018subject2vec}, which represents a volumetric image as an unordered set of patches. In addition, we introduce a multi-scale model which includes a conditional encoder for local textural and spatial feature extraction and a graph convolutional network for global contextual feature extraction. Our code will be made publicly available.

%which enable us to handle arbitrary sized images in full resolution. In addition, 
% In order to learn both local texture and global contextual features,
%In response to the COVID-19 pandemic, we show that 
In summary, we make the following contributions:
\begin{itemize}
\item We introduce a novel graph-based model with anatomical consistency for unsupervised representation learning, which enable us to handle arbitrarily sized images in full resolution.
\item We introduce a hierarchical model that can learn both local textural and global contextual features. The introduced interleaving training scheme that can significantly reduce memory footprint for end-to-end training.
\item We propose a task-specific model visualization method that can identify discriminative image regions.
\item We evaluate our method by extensive experiments on different datasets. The proposed method offers significant improvements over the baseline methods.
\end{itemize}

%Unsupervised Representation Learning with Graph-based Multi-scale 

==> method.tex <==
In this section, we first 
%provide a brief introduction on contrastive learning. Then, we 
introduce our method on graph representation of volumetric images, followed by the introduction of the proposed multi-scale model. Next we introduce the proposed model explanation method. We conclude this section with the optimization scheme and the implementation details. Our method is summerized in Fig.~\ref{fig:main}.

\begin{figure*}[t]
\centering
    \includegraphics[width = .9\textwidth]
    {figures/SSL_Diagram_v2.png}
    %\caption{Overview of our method. Our model consists of conditional encoder (Orange) for local textural feature extraction and graph neural network (Green) for global contextual feature extraction. Orange box indicates features extracted for each patch. The detailed architecture of the networks are presented in \textbf{Supplementary Material}.
    \caption{\ky{Schematic diagram of the proposed method. Our self-supervised learning approach imposes anatomical correspondences among patients via registration and uses a graph neural network to incorporate the relationship between different anatomical regions. We introduce a novel approach that integrates two parallel self-supervised representation learning objectives. The first row illustrates the contrastive learning on the regional anatomical level (patch level), which uses a conditional encoder with both texture information and location information as inputs. The second row illustrates the other contrastive learning on the patient level (graph level), which uses a graph neural network with patient-specific adjacent matrix and patch level representations as inputs.}
    }
    \label{fig:main}
\end{figure*}
%\subsection{Background}
%To be finished.

\subsection{Anatomical consistent Graph Representation of Images}
We represent \ky{the} image of \ky{an} subject $X_i$ as a graph of volumetric patches extracted from the lung region $\mathcal{G}_i=(\mathcal{V}_i,\mathcal{E}_i)$, where $\mathcal{V}_i=\{x_i^j\}_{j=1}^{N}$ denotes \ky{the} set of patches that cover the lung region of patent $i$, $\mathcal{E}_i$ denotes the set of edges.  We use an adjacency matrix $A_i\in N \times N$ to represent $\mathcal{E}_i$, defined as:
  \begin{equation}
    A_i^{jk}=
    \begin{cases}
      1, & \text{if}\ dist(p_i^j, p_i^k) < \rho \\
      0, & \text{otherwise}
    \end{cases},
  \end{equation}
where $dist(\cdot,\cdot)$ denotes Euclidean distance; $p_i^j$ and $p_i^k\in \mathcal{R}^3$ denotes coordinate of center for patches $x_i^j$ and $x_i^k$, respectively; $\rho$ is the threshold hyper-parameter.

To ensure anatomical correspondence of each node (patch) across all subjects, we perform registration to transform images of every subject to an atlas image of selected healthy subject with ANTs~\cite{tustison2014large}, which aims to minimize 
\begin{equation}
Sim(\phi_i(X_i), X_{Atlas}) + Reg(\phi_i),
\end{equation}
where $Sim$ is the similarity metric, $\phi_i(\cdot)$ is the fitted transform, $Reg(\phi_i)$ is the regularization term. The center coordinate used to extract each patch is acquired by reversely apply the transform to the coordinates of center coordinate of patches on the atlas image, specifically $p_i^j=\phi_i^{-1}(p^j)$. In this way, each node (patch) across all subjects would capture the same anatomical region:
\begin{equation}
\phi_0(p_0^j) = \phi_1(p_1^j) = \ldots = \phi_i(p_i^j)  = p^j.
\end{equation}

\subsection{Learning Patch-level Local Representation }
The anatomical location of lesion plays a role in patents' survival outcome, and the distribution of lesions varies across different anatomical location in lung. In order to extract anatomy-specific local features, we adopt a conditional encoder  $E(\cdot,\cdot)$ that takes both patch $x_i^j$ and patch location $p_i^j$ as input. It is consisted of a CNN feature extractor $e_l(\cdot)$ and a MLP head $f_l(\cdot)$, thus we have the encoded patch-level feature:
\begin{equation}
h_i^j=f_l(e_l(x_i^j)\mathbin\Vert p^j),
\end{equation}
where $\mathbin\Vert$ denotes concatenation.

We adopts InfoNCE loss~\cite{oord2018representation}, a form of contrastive loss to train the conditional encoder on patch level:
\begin{equation}
\mathcal{L}_l=-\log\frac{exp(q_i^j\cdot k_{+}/\tau)}{exp(q_i^j\cdot k_{+}/\tau)+\sum_{k_{-}} exp(q_i^j\cdot k_{-}/\tau)},
\end{equation}
where $\tau$ denotes temperature hyper-parameter.

We form positive pairs by generating two randomly augmented patches of the same one, the negative sample is generated by random augmenting a patch of another subject at the same anatomical location, specifically:
\begin{align*}
q_i^j&=f_l(e_l(aug(x_i^j))\mathbin\Vert p^j),
\\
k_+&=f_l(e_l(aug(x_i^j))\mathbin\Vert p^j),
\\
k_-&=f_l(e_l(aug(x_v^j))\mathbin\Vert p^j), v\neq i.
\end{align*}


\subsection{Learning Graph-level Global Representation }
Based on the node (patch) level local representation discussed above, we summarize them into subject-level global representation with graph neural network (GCN)~\cite{duvenaud2015convolutional}. Specifically, $G(\cdot,\cdot)$ takes patch-level representation $H_i$ and adjacency matrix $A_i$ as input, and it first updates node-level features by using information from neighboring nodes: 
\begin{equation}
H'_i =\texttt{concat}(\{{h'}_i^j\}_{j=1}^N)= \sigma\left( \hat{D}_i^{-\frac{1}{2}}\hat{A}_i\hat{D}_i^{-\frac{1}{2}}H_iW\right) ,
\end{equation}
where $\hat{A}_i = A_i + I$, $I$ is the identity matrix, $\hat{D}_i$ is the diagonal node degree matrix of $\hat{A}_i$, $H=\texttt{concat}(\{h_i^j\}_{j=1}^N)$ is a $N\times F$ matrix containing features of all nodes for a certain subject, and $W$ is the weight matrix, $\sigma$ is the activation function.

Then we obtain subject-level representation by pooling features across the graph followed by a MLP head $f_g$:
\begin{equation}
S_i=f_g(Pool(H'_i))
\end{equation}

We adopt InfoNCE loss to train the GCN on subject level:
\begin{equation}
\mathcal{L}_g=-\log\frac{exp(q_i\cdot k_{+}/\tau)}{exp(q_i\cdot k_{+}/\tau)+\sum_{k_{-}} exp(q_i\cdot k_{-}/\tau)}.
\end{equation}
We form positive pairs by generating two randomly augmented all patches of the same subject, the negative sample is generated by random augmenting all patches of another subject, specifically:
\begin{align*}
q_i&=G(\texttt{concat}(\{E(aug(x_i^n), p^n)\}_{n=1}^N), A_i),
\\
k_+&=G(\texttt{concat}(\{E(aug(x_i^n), p^n)\}_{n=1}^N), A_i),
\\
k_-&=G(\texttt{concat}(\{E(aug(x_v^n), p^n)\}_{n=1}^N), A_v), v\neq i.
\end{align*}
\subsection{Overall Model}
The model is trained in an end-to-end fashion. To exploit both patch-level local representation and graph-level global representation, we define the overall loss function as:
\begin{equation}
    \mathcal{L}  =  \mathcal{L}_l(E) +  \mathcal{L}_g(G)
\end{equation}
Since directly backpropagating gradient from $\mathcal{L}_g(G)$ to parameters in conditional encoder $E$ is unfeasible due to excessive memory footprint used by large number of patches ($N=581$), we propose an interleaving algorithm to train the model:
\begin{algorithm}
\caption{Interleaving update algorithm}
\begin{algorithmic}
\REQUIRE Conditional encoder $E(\cdot,\cdot)$, GCN $G(\cdot,\cdot)$.
\FOR{step $t=1,T_{max}$}
    \FOR{step $t_l=1,T_{l}$}
        \STATE Randomly sample a batch of $B_l$ subjects
        \FOR{$j=1,N$}
             \STATE $h_i^j$ $\leftarrow$ $E(aug(x_i^j),p^j)$
             \STATE Update $E$ by backpropagating $\mathcal{L}_l$
        \ENDFOR
    \ENDFOR
    \FOR{step $t_g=1,T_{g}$}
        \STATE Randomly sample a batch of $B_g$ subjects
        \STATE $S_i$$\leftarrow$$G(\texttt{concat}(\{E(aug(x_i^n), p^n)\}_{n=1}^N), A_i)$
        \STATE Update $G$ by backpropagating $\mathcal{L}_g$
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Model Explanation}
Understanding how the model makes prediction is important to build trust in the system. In this section, we propose a method for task-specific explanation of prediction of the proposed method. Our method is expanded from class activation maps (CAM)~\cite{zhou2016learning}. Without loss of generality, we assume that a Logistic regression model is trained on frozen features for a downstream binary classification task. Then predicted probability of class variable $Y_i=1$ given subject-level features $S'_i$ can be written as:
\begin{equation}
p(Y_i=1|S'_i) = {\frac {1}{1+e^{-(\beta +WS'_i)}}},
\end{equation}
where $S'_i=Pool(H'_i)$, the MLP head $f_g$ is discarded when extracting features for downstream tasks following the practice in~\cite{chen2020simple,chen2020improved} and $\beta$ and $W$ are learnt parameters. By plugging $S'_i=\frac{1}{N}\sum_{j=1}^{N}{h'}_i^{j}$ into the logit $l=\beta +WS'_i$, we have
\begin{equation}
l=\beta +\frac{1}{N}\sum_{j=1}^{N}W{h'}_i^{j}.
\end{equation}
We define $M_i$ as the class activation graph for class $Y_i=1$, where element of each node $x_i^j$ is given by 
\begin{equation}
M_i^j=W{h'}_i^{j}.
\end{equation}

We can see that $l=\beta+\frac{1}{N}\sum_{j=1}^{N}M_i^j$, which implies that $M_i^j$ can be seen as the contribution of node (patch) $x_i^j$ to the logit $l$.

\subsection{Implementation Details}
We train the proposed model for 30 epochs. We let the learning rate to be $3\times10^{-2}$. We also employed momentum $= 0.9$ and weight decay $= 1\times10^{-4}$ in the Adam optimizer. The batch size at patch level and subject level are set as 128 and 16, respectively. We let the representation dimension $F$ be $128$. Following the practice in MoCo, we maintain a queue of data samples and use momentum update scheme to increase the number of negative samples in training, as shown in previous work it can improve performance on downstream task~\cite{he2020momentum}. The number of negative samples during traing is defined to be $4096$. The data augmentation setting include random elastic transform, adding random Gaussian noise and random contrast adjustment. The temperature $\tau$ is chosen to be $0.2$. There are $581$ patches per subject/graph. The experiments are performed on 2 GPUs, each with 16GB embedded memory. The detailed network architecture can be found in \textbf{Supplementary Material}.
 

==> related_work.tex <==
\subsection{Unsupervised Learning}
Unsupervised learning aims to learn meaningful representations without human annotated data. Most unsupervised learning methods can be classified into generative and discriminative approaches. Generative approaches learn the distribution of data and latent representation by generation. These methods include adversarial learning and autoencoder based methods,  However, generating data at pixel space can be computationally intensive, and generating fine detail may not be necessary for learning effective representation. 

Discriminative approaches uses pre-text tasks for representation learning. Compared with supervised approaches, both the inputs and labels are derived from an unlabeled dataset. Discriminative approaches can be grouped into (1) pre-text tasks based on heuristics, including solving jigsaw puzzles~\cite{noroozi2016unsupervised}, context predication~\cite{doersch2015unsupervised}, colorization~\cite{zhang2016colorful} and (2) contrastive methods. Among them contrastive methods achieve state-of-the-art performance in many tasks. The core idea of contrastive learning is to bring different views of the same image (called as 'positive pairs') closer, and spreading representations of views from different images (called as 'negative pairs'). The similarity is measured by dot product in feature space~\cite{wu2018unsupervised}. Previous works have suggested that the performance of contrastive learning relies on large batch size~\cite{chen2020simple} and number of negative samples~\cite{he2020momentum}. 

\subsection{Representation Learning for Graph}
Learning effective representation for arbitrarily structured graph can help discover novel or interesting structure, it is also important for understanding graph-level representation. A number of algorithms proposed to used random walk-based methods for unsupervised representation learning on graph~\cite{grover2016node2vec,perozzi2014deepwalk,hamilton2017inductive}. These methods are powerful but rely more on local neighbors than structural information~\cite{ribeiro2017struc2vec}. Graph convolutional networks (GCN)~\cite{duvenaud2015convolutional,kipf2016semi} are proposed to generalize convolutional neural networks to work on the graphs.
Recently, Deep Graph Infomax~\cite{velickovic2019deep} is proposed to learn node-level representation by maximizing mutual information between patch representations and corresponding high-level summaries of graphs.

==> sections/abstract_v1.tex <==
The success of supervised learning with deep neural networks heavily relies on large-scale annotated datasets. However, for medical image analysis, human annotation is time-consuming and expensive. Until now, very few annotated COVID-19 imaging datasets are publicly available, which hinders the development of AI solutions in response to the pandemic. In this work, we introduce a novel self-supervised approach for learning local and global features from volumetric medical images. We represent a volumetric medical image as a graph of locally connected patches with anatomical consistency across patients. Contrastive loss is used to learn region-specific features at the patch level and subject-specific features at the graph level. Since medical images of different patients have different sizes and spacing has a physical meaning, the graph representation has the advantage of handling any arbitrarily sized image in full resolution. We also introduce an interleaving scheme that alternates the training between node level and graph level, which significantly reduces the memory footprint for end-to-end training. Experiments on large-scale lung CT datasets show that our approach compares favorably to baseline methods. We also demonstrate that representations learnt can be used to quantify the clinical progression of COVID-19 and transferred well to COVID-19 patients from different hospitals. Qualitative results suggest that our model can identify clinical-relevant regions in the images.
%for COVID-19 image classification. Model visualization results indicate that our model focus on clinical-relevant image regions.
%The success of supervised learning with deep neural network \ky{heavily} relies on large-scale annotated datasets. However\ky{,} for medical image analysis, human annotation is time-consuming and expensive. \ky{It is usually easier to access a large number of unlabelled medical images rather than a large number of annotated medical images. Self-supervised learning exploiting inherent anatomical information from raw data is an appealing solution to this problem. In this work, we introduce a novel self-supervised approach for learning hierarchical features from volumetric medical images. We represent a volumetric medical image as a graph of locally connected 3D patches, obtain region-specific anatomical features through contrastive learning at the node level, and obtain subject-specific features through contrastive learning at the graph level. Since medical images of different patients have different sizes, the graph representation has the advantage of handling any arbitrarily sized image in full resolution. We also introduce an interleaving scheme that alternates the training between node level and graph level, which significantly reduces the memory footprint for end-to-end training. Our experiment on a large-scale lung CT data set of Chronic Obstructive Pulmonary Disease (COPD) shows that our approach compares favorably to other unsupervised baselines, and even outperforms supervised methods on predicting some of the physiologic measures. More importantly, we demonstrate that the representations of lung CT scans learned by our approach is useful in quantifying COVID-19 progression and transfers well to diagnosing COVID-19 in a cohort of patients from multiple hospitals. }
%introduce a novel graph-based network unsupervised representation learning on volumetric medical images. Since medical images are of variable dimensions and spacing has \ky{a} physical meaning, we propose (1) to represent \ky{a volumetric} image as a graph of \ky{3D} patches 
% with anatomical \ky{consistency, }%consistence which enable us to handle arbitrary sized images in full resolution\ky{,} (2) a hierarchical model to extract \ky{both local and global anatomical features, }
%local textural and global contextual features \ky{and }(3) an interleaving training scheme that can significantly reduce memory footprint for end-to-end training \ky{on volumetric medical images}. Experiments on \ky{a} large-scale 3D thorax CT datasets demonstrate that our approach outperforms baseline methods. Model visualization results indicate that our model can localize discriminative image regions.

==> sections/method_v2.tex <==
\ky{In this section, we first introduce our method of graph representation of volumetric images. We then introduce our graph-based contrasting learning objectives, one at the node level and another at the graph level. Next, we introduce the proposed model explanation method. We conclude this section with the optimization scheme and the implementation details. Our method is summarized in Fig.~\ref{fig:main}.}

%\ky{In this section, we first introduce our graph representation of medical images. We then introduce the proposed self-supervised learning approach based on the multi-scale model.}

\begin{figure*}[htp]
\centering
    \includegraphics[width = \textwidth]
    {figures/SSL_Diagram_v8.png}
    %\caption{Overview of our method. Our model consists of conditional encoder (Orange) for local textural feature extraction and graph neural network (Green) for global contextual feature extraction. Orange box indicates features extracted for each patch. The detailed architecture of the networks are presented in \textbf{Supplementary Material}.
    \caption{Schematic diagram of the proposed method. Our self-supervised learning approach imposes anatomical correspondences among patients via registration and uses a graph neural network to incorporate the relationship between different anatomical regions. We introduce a novel approach that integrates two parallel self-supervised representation learning objectives. 
    %The orange box illustrates the contrastive learning on the patch level, which uses a conditional encoder with both texture information and location information as inputs. The green box illustrates the other contrastive learning on the graph level, which uses a graph neural network with subject-specific adjacent matrix and patch level representations as inputs.
    }
    \label{fig:main}
\end{figure*}
%\subsection{Background}
%To be finished.

\subsection{Anatomical Consistent Graph Representation of Images}
Since people have lungs with different shapes and sizes, we first perform image registration to ensure anatomical correspondence across all subjects. 
We use image registration to find the correspondences between anatomical landmarks of the patients. We choose the image of a healthy subject as the atlas image $X_{\text{Atlas}}$, and align the image $X_i$ of each other subject with respect to $X_{\text{Atlas}}$. We use the ANTs software~\cite{tustison2014large} that minimizes the following loss function to find the correspondences in an unsupervised way:
\begin{equation}
Sim(\phi_i(X_i), X_{\text{Atlas}}) + Reg(\phi_i),
\end{equation}
where $Sim$ is a similarity metric (e.g., $\ell_2$ norm), $\phi_i(\cdot)$ is the fitted subject-specific transformation, $Reg(\phi_i)$ is a regularization term to ensure the transformation is smooth enough.

To define a standard set of anatomical regions, we divide the atlas image into a set of equally spaced 3D patches $\{x^j\}_{j=1}^{N}$ with some overlap, where $j$ is the index for the anatomical region, and $N$ denotes the total number of anatomical regions in the lung. We obtain the center coordinates of the corresponding anatomical regions on the other images by using the inverse transform $p_i^j=\phi_i^{-1}(p_\text{Atlas}^j)$, where $p_\text{Atlas}^j$, $p_i^j$ denotes the center coordinates of patch $j$ on the atlas image and the image of the subject $i$ respectively. In this way, patches with the same index across all subjects map to the same anatomical region on the atlas image:
\begin{equation}
\phi_1(p_1^j) = \phi_2(p_2^j) = \ldots = \phi_i(p_i^j)  = p_\text{Atlas}^j
\end{equation}

To incorporate the relationship between different anatomical regions, we represent an image as a graph of patches (nodes), whose edge connectivity is determined by the Euclidean distance between patches' centers. More formally, the image $X_i$ is represented as $\mathcal{G}_i=(\mathcal{V}_i,\mathcal{E}_i)$, where $\mathcal{V}_i=\{x_i^j\}_{j=1}^{N}$ denotes the set of patches that cover the lung region of subject $i$, and $\mathcal{E}_i$ denotes the set of edges. We use an adjacency matrix $A_i\in N \times N$ to represent $\mathcal{E}_i$, defined as:
  \begin{equation}
    A_i^{jk}=
    \begin{cases}
      1, & \text{if}\ \text{dist}(p_i^j, p_i^k) < \rho \\
      0, & \text{otherwise}
    \end{cases},
  \end{equation}
where $\text{dist}(\cdot,\cdot)$ denotes the Euclidean distance; $p_i^j$ and $p_i^k\in \mathcal{R}^3$ are the coordinates of centers in patches $x_i^j$ and $x_i^k$, respectively; $\rho$ is the threshold hyper-parameter that controls the density of graph.

\subsection{Learning Patch-level Representation }
Anatomy provides important context for identifying abnormal tissues in medical imaging analysis. For a given anatomical region, a desirable method should be sensitive enough to  detect  deviation  from normal-appearing  tissue.
In addition, the anatomical location of lesion plays a role in patents' survival outcome, and the %distribution of lesions
 types of lesion
%shape and texture }
vary across different anatomical locations in lung. In order to extract anatomy-specific features, we adopt a conditional encoder  $E(\cdot,\cdot)$ that takes both patch $x_i^j$ and patch location $p_i^j$ as input. It is \ky{composed with} a CNN feature extractor $C(\cdot)$ and a MLP head $f_l(\cdot)$, thus we have the encoded patch-level feature:
\begin{equation}
h_i^j=E(x_i^j, p_i^j)=f_l(C(x_i^j)\mathbin\Vert p_\text{Atlas}^j)),
\end{equation}
where $\mathbin\Vert$ denotes concatenation, .

We adopt the InfoNCE loss~\cite{oord2018representation}, a form of contrastive loss to train the conditional encoder on the patch level:
\begin{equation}
\mathcal{L}_l=-\log\frac{\exp(q_i^j\cdot k_{+}/\tau)}{\exp(q_i^j\cdot k_{+}/\tau)+\sum_{k_{-}} \exp(q_i^j\cdot k_{-}/\tau)},
\end{equation}
where $q_i^j$ denotes the representation of query patch $x_i^j$, $k_{+}$ and $k_{-}$ denotes the representation of the positive and the negative key respectively, and $\tau$ denotes the temperature hyper-parameter. We obtain a positive sample pair by generating two randomly augmented views 
%of the same one,
from the same query patch $x_i^j$,
and obtain a negative sample by augmenting the patch $x_v^j$ at the same anatomical region $j$ from a random subject $v$,
%patch of another subject at the same anatomical location, 
specifically:
\begin{align*}
q_i^j&=f_l(C(aug(x_i^j))\mathbin\Vert p_\text{Atlas}^j),
\\
k_+&=f_l(C(aug(x_i^j))\mathbin\Vert p_\text{Atlas}^j),
\\
k_-&=f_l(C(aug(x_v^j))\mathbin\Vert p_\text{Atlas}^j), v\neq i.
\end{align*}


\subsection{Learning Graph-level Representation }
We adopt the Graph Convolutional Network (GCN)~\cite{duvenaud2015convolutional} to summarize the patch-level \ky{(anatomy-specific)} representation into the graph-level \ky{(subject-specific)} representation. We consider each patch as one node in the graph, and the subject-specific adjacent matrix determines the connection between nodes.
Specifically, the GCN model $G(\cdot,\cdot)$ takes patch-level representation $H_i$ and adjacency matrix $A_i$ as inputs, and propagates information across the graph to update node-level features:
%it first updates node-level features by using information from neighboring nodes: 
\begin{equation}
H'_i =\texttt{concat}(\{{h'}_i^j\}_{j=1}^N)= \sigma\left( \hat{D}_i^{-\frac{1}{2}}\hat{A}_i\hat{D}_i^{-\frac{1}{2}}H_iW\right) ,
\end{equation}
where $\hat{A}_i = A_i + I$, $I$ is an identity matrix, $\hat{D}_i$ is a diagonal node degree matrix of $\hat{A}_i$, $H_i=\texttt{concat}(\{h_i^j\}_{j=1}^N)$ is a $N\times F$ matrix containing $F$ features for all $N$ nodes in the image of the subject $i$, and $W$ is a learnable projection matrix, $\sigma$ is a nonlinear activation function.

Then we obtain subject-level representation by global average pooling all nodes in the graph followed by a MLP head $f_g$:
\begin{equation}
S_i=f_g(\texttt{Pool}(H'_i))
\end{equation}

We adopt the InfoNCE loss to train the GCN on the graph level:
\begin{equation}
\mathcal{L}_g=-\log\frac{\exp(r_i\cdot t_{+}/\tau)}{\exp(r_i\cdot t_{+}/\tau)+\sum_{t_{-}} \exp(r_i\cdot t_{-}/\tau)}.
\end{equation}
where $r_i^j$ denotes the representation of the entire image $X_i$, $t_{+}$ and $t_{-}$ denotes the representation of the positive and the negative key respectively, and $\tau$ denotes the temperature hyper-parameter.
To form a positive pair, we take two views of the same image $X_i$ under random augmentation at patch level. We obtain a negative sample by randomly sample a different image $X_v$, specifically:
\begin{align*}
r_i&=G(\texttt{concat}(\{E(aug(x_i^n), p_\text{Atlas}^n)\}_{n=1}^N), A_i),
\\
t_+&=G(\texttt{concat}(\{E(aug(x_i^n), p_\text{Atlas}^n)\}_{n=1}^N), A_i),
\\
t_-&=G(\texttt{concat}(\{E(aug(x_v^n), p_\text{Atlas}^n)\}_{n=1}^N), A_v), v\neq i.
\end{align*}

\subsection{Overall Model}
The model is trained in an end-to-end fashion by integrating the two InfoNCE losses obtained from patch level and graph level.
%The model is trained in an end-to-end fashion. To exploit both patch-level local representation and graph-level global representation, 
We define the overall loss function as follows:
\begin{equation}
    \mathcal{L}  =  \mathcal{L}_l(E) +  \mathcal{L}_g(G)
\end{equation}
Since directly backpropagating gradients from $\mathcal{L}_g(G)$ to the
parameters in the conditional encoder $E$ is unfeasible due to the excessive memory footprint accounting for a large number of patches, we propose an interleaving algorithm that alternates the training between patch level and graph level to solve this issue. \ky{The algorithmic description of the method is shown below.}
\begin{algorithm}
\caption{Interleaving update algorithm}
\begin{algorithmic}
\REQUIRE Conditional encoder $E(\cdot,\cdot)$, GCN $G(\cdot,\cdot)$.
\FOR{step $t=1,T_{max}$}
    \FOR{step $t_l=1,T_{l}$}
        \STATE Randomly sample a batch of $B_l$ subjects
        \FOR{$j=1,N$}
             \STATE $h_i^j$ $\leftarrow$ $E(aug(x_i^j),p^j)$
             \STATE Update $E$ by backpropagating $\mathcal{L}_l$
        \ENDFOR
    \ENDFOR
    \FOR{step $t_g=1,T_{g}$}
        \STATE Randomly sample a batch of $B_g$ subjects
        \STATE $S_i$$\leftarrow$$G(\texttt{concat}(\{E(aug(x_i^n), p^n)\}_{n=1}^N), A_i)$
        \STATE Update $G$ by backpropagating $\mathcal{L}_g$
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Model Explanation}
Understanding how the model makes predictions is important to build trust in medical imaging analysis. In this section, we propose a method that provides task-specific explanation for the predicted outcome.
% of the proposed method. 
Our method is expanded from the class activation maps (CAM) proposed by~\cite{zhou2016learning}. 
Without loss of generality, we assume a Logistic regression model is fitted
%\ky{In particular, 
for a downstream binary classification task on the extracted subject-level features $S'_i$, the predicted probability of dependent variable $Y_i=1$ for subject $i$ can be written as:
\begin{equation}
%\bm{p}(Y_i=1|S'_i) = {\frac {1}{1+e^{-(\beta +WS'_i)}}},
\log \frac{\mathbb{P}(Y_i = 1 | S'_i) }{\mathbb{P}(Y_i = 0 | S'_i) } = \beta+WS'_i=\beta+ \sum_{j=1}^{N}\underbrace{  W h_{i}'^j }_{M_i^j}
\end{equation}
where $S'_i=\texttt{Pool}(H'_i)$, the MLP head $f_g$ is discarded when extracting features for downstream tasks following the practice in~\cite{chen2020simple,chen2020improved}, and $\beta$ and $W$ are the learned logistic regression weights. By plugging $S'_i=\frac{1}{N}\sum_{j=1}^{N}{h'}_i^{j}$ into the logit $l_i=\beta +WS'_i$, we have
\begin{equation}
l_i=\beta +\frac{1}{N}\sum_{j=1}^{N}W{h'}_i^{j}.
\end{equation}
We define $M_i$ as the class activation graph for the subject $i$, in which
\begin{equation}
M_i^j=W{h'}_i^{j}.
\end{equation}
%can be viewed as the contribution from the anatomical region $j$ to the predicted outcome of subject $i$.
We can see that $l_i=\beta+\frac{1}{N}\sum_{j=1}^{N}M_i^j$, which implies that $M_i^j$ can be viewed as the contribution of anatomical region $x_i^j$ to the logit $l_i$.

\subsection{Implementation Details}
We train the proposed model for 30 epochs. We set the learning rate to be $3\times10^{-2}$. We also employed momentum $= 0.9$ and weight decay $= 1\times10^{-4}$ in the Adam optimizer. The batch size at patch level and subject level is set as 128 and 16, respectively. We let the representation dimension $F$ be $128$. Following the practice in MoCo, we maintain a queue of data samples and use a momentum update scheme to increase the number of negative samples in training; as shown in previous work, it can improve performance of downstream task~\cite{he2020momentum}. The number of negative samples during training is set as $4096$. The data augmentation includes random elastic transform, adding random Gaussian noise, and random contrast adjustment. The temperature $\tau$ is chosen to be $0.2$. There are $581$ patches per subject/graph. The experiments are performed on 2 GPUs, with 16GB memory in each. The detailed network architecture can be found in \textbf{Supplementary Material}.
 
